Latticed $k$-Induction with an Application to Probabilistic Programs

We revisit two well-established verification techniques, $k$-induction and bounded model checking (BMC), in the more general setting of fixed point theory over complete lattices. Our main theoretical contribution is latticed $k$-induction, which (i) generalizes classical $k$-induction for verifying transition systems, (ii) generalizes Park induction for bounding fixed points of monotonic maps on complete lattices, and (iii) extends from naturals $k$ to transfinite ordinals $\kappa$, thus yielding $\kappa$-induction. The lattice-theoretic understanding of $k$-induction and BMC enables us to apply both techniques to the fully automatic verification of infinite-state probabilistic programs. Our prototypical implementation manages to automatically verify non-trivial specifications for probabilistic programs taken from the literature that - using existing techniques - cannot be verified without synthesizing a stronger inductive invariant first.

==> app-kind-cex.tex <==
\subsection{Counterexample regarding Remark~\ref{rem:kind_sat_req}}
Consider the transition system $\transsys = (\stateset,\, \init, \transrel)$ with $\stateset = \{s_1, s_2\} = \init$ and $\transrel=\emptyste$.

==> benchmarks.tex <==
\begin{figure}
   \begin{tabular}{llrrrr}
   	\toprule
   	name &             status & k &  compute\_formulae\_time &  sat\_check\_time &  total\_time \\
   	\midrule
   	2drwalk &   TO & / &                      / &               / &           / \\
   	bayesian\_network &   TO & / &                      / &               / &           / \\
   	ber &  inductive & 1 &                   0.01 &            0.00 &        0.09 \\
   	C4B\_t303 &  inductive & 3 &                   0.09 &            0.01 &        0.22 \\
   	condand &  inductive & 1 &                   0.01 &            0.00 &        0.08 \\
   	fcall &  inductive & 1 &                   0.01 &            0.00 &        0.08 \\
   	hyper &  inductive & 1 &                   0.01 &            0.00 &        0.09 \\
   	linear01 &  inductive & 1 &                   0.01 &            0.00 &        0.08 \\
   	prdwalk &  inductive & 1 &                   0.01 &            0.00 &        0.20 \\
   	prspeed &  inductive & 1 &                   0.01 &            0.00 &        0.15 \\
   	race &  inductive & 1 &                   0.01 &            0.00 &        0.75 \\
   	rdspeed &  inductive & 1 &                   0.01 &            0.00 &        0.15 \\
   	rdwalk &  inductive & 1 &                   0.01 &            0.00 &        0.08 \\
   	sprdwalk &  inductive & 1 &                   0.01 &            0.00 &        0.08 \\
   	\bottomrule
   \end{tabular}

    \begin{tabular}{llrrrr}
    	\toprule
    	name &             status &  k &  compute\_formulae\_time &  sat\_check\_time &  total\_time \\
    	\midrule
    	brp1 &  inductive &  5 &                   0.17 &            0.01 &        0.29 \\
    	brp2 &  inductive & 11 &                   1.73 &            0.11 &        1.98 \\
    	brp3 &  inductive & 23 &                  17.77 &           29.18 &       47.12 \\
    	brp4 &   TO &  / &                      / &               / &           / \\
    	brp5 &   refuted & 13 &                   0.85 &           14.51 &       15.40 \\
    	brp6 &   TO &  / &                      / &               / &           / \\
    	brp7 &   TO &  / &                      / &               / &           / \\
    	geo1 &  inductive &  2 &                   0.01 &            0.00 &        0.08 \\
    	geo2 &   refuted & 46 &                   0.43 &            0.05 &        0.54 \\
    	geo3 &   refuted & 11 &                   0.05 &            0.01 &        0.10 \\
    	rabin1 &  inductive &  1 &                   0.01 &            0.00 &        0.16 \\
    	rabin2 &  inductive &  5 &                   1.35 &            0.03 &        1.55 \\
    	rabin3 &   TO &  / &                      / &               / &           / \\
    	rabin4 &   refuted &  4 &                   0.32 &            0.03 &        0.41 \\
    	rabin5 &   refuted &  8 &                   8.12 &            2.82 &        11.5 \\
    	unif\_gen1 &  inductive &  2 &                   0.27 &            0.02 &        0.60 \\
    	unif\_gen2 &  inductive &  3 &                   1.58 &            0.10 &        1.96 \\
    	unif\_gen3 &  inductive &  3 &                   1.55 &            0.12 &        1.94 \\
    	unif\_gen4 &  inductive &  5 &                  49.69 &           16.68 &       66.64 \\
    	unif\_gen5 &   TO &  / &                      / &               / &           / \\
    	\bottomrule
    \end{tabular}
    \caption{Experimental results. started/started = TO = 15 min.}
\end{figure}



==> bmc.tex <==
%
Given a countable set of $\Nats$-valued arithmetic expressions $\aexp$ and a countable set of Boolean expressions $\bexp$, we denote by $\pgclparam{\aexp}{\bexp}$ the set of single-loop programs $\cc$ adhering to the grammar
%
%
\begin{align*}
	\cc \qqlongrightarrow  &\WHILEDO{\bb}{\cc'} \tag{while loop} \\
	%
	\phantom{aa} \\
	%
	\cc' \qqlongrightarrow 	
	%
	%
	& \SKIP	\tag{effectless program} \\
	%
	& \qmid  \ASSIGN{x}{\ee}  \tag{assignment}\\
	%
	& \qmid \COMPOSE{\cc'}{\cc'} \tag{sequential composition}\\
	%
	& \qmid  \PCHOICE{\cc'}{p}{\cc'} \tag{probabilistic choice}\\
	%
	& \qmid  \ITE{\bb}{\cc'}{\cc'}~, \tag{conditional choice}
	%
\end{align*}
%
where
%
%\begin{itemize}
%\item 
$x \in \Vars$ is a program variable,
%
%\item 
$\ee \in \aexp$ is an arithmetic expression,
%
%\item 
$p \in [0,1] \cap \Rats$ is a rational probability, and
%
%\item 
$\bb \in \bexp$ is a Boolean expression also referred to as \emph{guard}. 
%
%
%
Given a computable set $\SyntE$ of expectations, a computable set $\aexp$ of arithmetic expressions, and a computable set $\bexp$ of Boolean expressions, we call
%
\[
   \propspacesymb \eeq \propspace{\SyntE}{\pgclparam{\aexp}{\bexp}}
\]
%
a \emph{property space}. For $\ff, \fg \in \SyntE$ and $\cc \in \pgclparam{\aexp}{\bexp}$ we call a triple
%
\[
   \prop{\cc}{\ff}{\fg}
\]
%
a \emph{$\propspacesymb$-property}. We say that a $\propspacesymb$-property $\prop{\cc}{\ff}{\fg}$ \emph{holds} if 
%
\[
   \wp{\cc}{\ff} \lleq \fg~.
\]
%
Otherwise, we say that $\prop{\cc}{\ff}{\fg}$ \emph{does not hold}.

\subsection{BMC for Probabilistic Programs}


\begin{definition}
	Let $\propspacesymb = \propspace{\SyntE}{\pgclparam{\aexp}{\bexp}}$ be a property space. We say that
	%
	%\begin{itemize}
	%\item
	$\propspacesymb$ \emph{admits bounded model checking (admits BMC)}, if the set 
	%
	\[
	\left\{ (\cc, \ff, \fg) ~\mid~ (\cc, \ff, \fg)~\text{is a $\propspacesymb$-property that does not hold}~ \right\}
	\]
	%
	is semi-decidable. \hfill $\triangle$
	%\end{itemize}
\end{definition}
%
We are interested in sufficient conditions for admissibility of BMC.
%
\kbcommentinline{Somehow make clear that there must be an algorithm computing the expectations from (1)-(3)}
\begin{theorem}
	\label{thm:admissibility_bmc}
	A property space $\propspacesymb = \propspace{\SyntE}{\pgclparam{\aexp}{\bexp}}$ admits BMC, if 
	%
	\begin{enumerate}
		\item \label{thm:admissibility_bmc_1} $\SyntE$ is closed under substitution w.r.t.\ $\aexp$, i.e.,
		%
		\[
		    \forall \ff \in \SyntE ~ \forall \ee \in \aexp ~ \forall x \in \Vars \colon \quad  \ff\subst{x}{e} \in \SyntE~,
		\]
		%
		\item \label{thm:admissibility_bmc_2} $\SyntE$ is closed under guarding w.r.t.\ $\bexp$, i.e,
		\[
		     \forall \ff \in \SyntE ~ \forall \bb \in \bexp   \colon \quad \iverson{\bb} \cdot \ff \in \SyntE~,
	    \]
	    %
	    \item \label{thm:admissibility_bmc_3} $\SyntE$ is closed under convex sums, i.e.,
	    %
	    \[
	       \forall \ff, \fg \in \SyntE ~\forall p,q \in \PosRats \colon \quad p \cdot \ff + q \cdot \fg \in \SyntE, ~\text{and}
	    \]
	    %
	    \item \label{thm:admissibility_bmc_4} quantitative entailment in $\SyntE$ is decidable, i.e., for $\ff,\fg \in \SyntE$, it is decidable whether
	    %
	    \[
	          \ff \lleq \fg ~,
	    \]
	\end{enumerate}
	%
	and if furthermore there is an algorithm that computes the expectations from~\eqref{thm:admissibility_bmc_1}-\eqref{thm:admissibility_bmc_3}.
\end{theorem}
%
\begin{proofidea}
	%
	Let $\prop{\cc}{\ff}{\fg}$ with $\cc = \WHILEDO{\bb}{\cc'}$ be a $\propspacesymb$-property that does not hold.  By Lemma~\ref{lem:wp_klenee} there is an $n \geq 1$ with  $\charwpn{\bb}{\cc'}{\ff}{n}(0) \not\leq \fg$. Now, \eqref{thm:admissibility_bmc_1}-\eqref{thm:admissibility_bmc_3} imply that $\SyntE$ is closed under $\wp{\cc''}{\cdot} $ for all loop-free $\cc''$. Hence, $\charwpn{\bb}{\cc'}{\ff}{n}(0)$ is an element of $\SyntE$ and computable for every $n \geq 1$.
	Finally, since quantitative entailment in $\SyntE$ is decidable, Algorithm~\ref{alg:bmc} is the sought-after semi decision procedure.
    %
\end{proofidea}


==> bmc_algorithm.tex <==
	\begin{algorithm}[t]
		%\setstretch{2}
		\caption{Latticed bounded model checking}
		\label{alg:bmc}
		\SetKwInput{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
		\Input{$\laop\colon \laset \to \laset$ and $\laf \in \laset$.}
        \Output{\enquote{$\refute$} if there exists $k \in \Nats$ with $\lappup{k}{\bot} \not\laord \laf$, diverge otherwise.}
		%
		$\lag \leftarrow \bot$ \;
		%
		\Repeat{$\lag \not\laord \laf~$}{
			%
            $\lag \leftarrow \lapp{\lag}$ \;
			%
		}
		%
		%
		\Return $\refute$ \;
		%
	\end{algorithm}


==> challenges.tex <==
%\section{Current Challenges}
%%
%\begin{enumerate}
%	%
%	\item Investigate the quantifier-free SMT encoding. (See Section~\ref{sec:smt_encoding_example}) Is it sound? If not, can we fix it?
%	%
%	\item Set up a Python 3.7 project for implementing our BMC approach. We will use the solver agnostic library PySMT\footnote{\url{https://github.com/pysmt/pysmt}} to communicate with SMT solvers.
%	%
%	\item Precisely specify which input programs and expectations we allow for. Enable parsing these and think about appropriate data structures to represent (the abstract syntax tree of) $\pgcl$ programs and expectations.
%	%
%	\item Automatically compute the $\wpsymbol$-characteristic functional in summation normal form.
%	%
%	\item Apply an appropriate preprocessing to mittigate the exponential blow-up (cf.\ end of Section~\ref{sec:smt_encoding_example}).
%	%
%	\item Implement the BMC Approach. How feasible?
%	%
%	\item Invariant generation via craig interpolation. What can off-the-shelf craig interpolants do for us? 
%	%
%	\item (What can $k$-induction do for us? What does it even mean in the probabilistic setting?).
%\end{enumerate}

==> decidability_old.tex <==
We rely on the \emph{summation normal form (SNF)}:

\begin{lemma}
	\label{lem:dnf}
	Let $\ff \in \Elin$. There exist: 
	%
	\begin{enumerate}
		\item  A natural number $n\geq 1$,
		%
		\item  linear Boolean expressions $\bb_1,\ldots,\bb_n \in \bexplinq$, 
		%
		\item extended linear arithmetic expression $\eeinfty_1,\ldots,\eeinfty_n \in  \extaexplinq$ 
		%
		%\item non-negative rationals $\rr_1,\ldots,\rr_n \in \PosRats$
	\end{enumerate}
   %
   such that $\ff$ is equivalent to an effectively constructible linear expectation $\snf{\ff}$ in \emph{summation normal form}
	%6
	\[
	    \snf{\ff} \ddefeq \sum\limits_{i=1}^{n} \iverson{\bb_i} \cdot \eeinfty_i ~.
	\]
	%
	Furthermore, $\ff$ is equivalent to an effectively constructible expectation $\dnf{\ff}$ in \emph{disjunctive normal form} given by
	%
	\[
	     \dnf{\ff} \ddefeq \sum\limits_{i=1}^{m} \iverson{\bp_i} \cdot \eainfty_i ~,
	\]
	%
	which is an expectation in summation normal form where additionally the $\bp_i$ partition the state space, i.e., for every $\sigma \in \States$ there is \emph{exactly one} $i \in \{1,\ldots,m\}$ with $\bp_i(\sigma) = 1$.   %For $k\in \Nats$, write $\onetoarg{k} \defeq \{1,\ldots,k\}$.
	%
\end{lemma}
%
\begin{proof}
	%
	For $\snf{\ff}$, we proceed by induction on the structure of linear expectations (cf.\ \cite[Lemma A.2]{relatively_complete_prob_progs}).  We construct $\dnf{\ff}$ from $\snf{\ff}$ by 
	%
	\begin{align*}
		&\sum_{((\br_1, \eoinfty_1),\ldots,(\br_n, \eoinfty_n)) \in \bigtimes_{i=1}^n \{(\bb_i, \eeinfty_i), (\neg \bb_i, 0) \}}  \big[ \bigwedge_{i=0}^n \br_i \big] 
		\cdot 
		\begin{cases}
			\infty, & \text{if $\eoinfty_j = \infty$ for some $j$} \\
			%
			\sum_{i=1}^n \eoinfty_i, & \text{otherwise}~.
		\end{cases}
	\end{align*}
    %
\end{proof}
%
%
We show that quantitative entailment $\ff \leq \fg$ in $\Elin$ is decidable by reducing to satisfiability of quantifier-free mixed integer real arithmetic (\qflira) formulae, which is decidable \textcolor{red}{[CITE]}. Let $\ff, \fg \in \Elin$ with corresponding SNFs
%
\begin{align*}
	%
	\snf{\ff} \eeq \sum\limits_{i=1}^{n} \iverson{\bb_i}\cdot \eeinfty_i 
	%
	\qquad
	\text{and}
	\qquad
	%
	\snf{\fg} \eeq& \sum\limits_{i=1}^{m} \iverson{\bp_i}\cdot \eainfty_i ~.
\end{align*}
%
%
By Lemma~\ref{lem:dnf}, we have
%
%
\[
   \ff \lleq \fg \qquad \text{iff} \qquad \snf{\ff} \lleq \snf{\fg}~.
\]
%
%
%
Now let $\smtinfty$ be a fresh, unconstrained $\Nats$-valued SMT variable. 
For every extended linear arithmetic expression $\eeinfty$, define
%
\[
\tosmt{\eeinfty} \ddefeq
%
\begin{cases}
	%
	\smtinfty, & \text{if}~ \eeinfty = \infty \\
	%
	\eeinfty, & \text{if}~ \eeinfty \neq \infty~.
\end{cases}
%
\]
%
Next, we introduce $n+1$ (resp.\ $m+1$) $\Reals$-valued solver variables $x_0,\ldots,x_n$ (resp.\ $y_0,\ldots, y_m$) and construct the formula
%
\begin{align*}
	& x_0 = 0 \wwedge\bigwedge_{i=1}^n 
	     (\neg\bb_i \implies x_i = x_{i-1})
	     \wedge
	     (\bb_i \implies x_i = x_{i-1} + \tosmt{\eeinfty}) \\
    %
	\wwedge & y_0 = 0 \\
	%
	 \wwedge&\bigwedge_{i=1}^m 
	(\neg\bp_i \implies y_i = y_{i-1})
	\wedge
	(\bp_i \implies y_i = y_{i-1} +
		 \begin{cases}
		 	0, &\text{if}~\eeinfty=\infty \\
		 	%
		\tosmt{\eainfty_i}, & \text{otherwise}~,
		\end{cases} \\
	%
	\wwedge& x_n > y_m~.
\end{align*}
%
where we implicitly identify every occurring program variable in $\Vars$ by an $\Nats$-valued solver variable. The above formula is unsatisfiable iff $\ff \leq \fg$.
%
%We now define the effectively constructible \qflira formula
%%
%\begin{align*}
%	&\smtentails{\ff}{\fg} \\
%	%
%	 \ddefeq &
%	\bigvee_{i=1}^n 
%		\bigvee_{\substack{j=1 \\ \tosmt{\eainfty} \neq \infty}}^m 
%			(\bb_i \wwedge\bp_j 
%					\wwedge               \tosmt{\eeinfty_i}       >       \tosmt{\eainfty_j}
%			) ~,
%\end{align*}
%%
%where we implicitly identify every occurring program variable in $\Vars$ by an $\Nats$-valued SMT variable. 
%%
%Satisifiability of $\smtentails{\ff}{\fg}$ and the validity of $\ff \leq \fg$ are then related as follows:
%%
%\begin{align*}
%  %
%   &\ff \leq \fg \\
%   %
%   %
%   \text{iff} \qquad &  \dnf{\ff} \leq \dnf{\fg} 
%   \tag{by Lemma~\ref{lem:dnf}} \\
%   %
%   %
%   \text{iff} \qquad & \bigwedge_{i=1}^n \big( \iverson{\bb_i} \cdot \eeinfty_i \leq \sum\limits_{i=1}^{m} \iverson{\bp_i}\cdot \eainfty_i \big) 
%   \tag{the $\bb_i$ partition the state space}
%   \\
%   %
%   %
%   \text{iff} \qquad & \bigwedge_{i=1}^n \, \bigwedge_{j=1}^m  \iverson{\bb_i} \cdot \eeinfty_i \leq  \iverson{\bp_j}\cdot \eainfty_j 
%   \tag{the $\bp_j$ partition the state space}\\
%   %
%   %
%   \text{iff} \qquad & \bigwedge_{i=1}^n \, \bigwedge_{\substack{j=1 \\ \tosmt{\eainfty_j} \neq \infty}}^m \iverson{\bb_i} \cdot \eeinfty_i \leq  \iverson{\bp_j}\cdot \eainfty_j 
%   \tag{nothing is greater than $\infty$}\\
%   %
%   %
%   \text{iff} \qquad & \forall \pstate \in \States \colon \bigwedge_{i=1}^n \, \bigwedge_{\substack{j=1 \\ \tosmt{\eainfty_j} \neq \infty}}^m (\iverson{\bb_i} \cdot \eeinfty_i)(\pstate) \leq  (\iverson{\bp_j}\cdot \eainfty_j)(\pstate) 
%   \tag{$\leq$ on expectations is defined point-wise}\\
%   %
%   %
%   \text{iff} \qquad & \neg\exists \pstate \in \States \colon \bigvee_{i=1}^n \, \bigvee_{\substack{j=1 \\ \tosmt{\eainfty_j} \neq \infty}}^m (\iverson{\bb_i} \cdot \eeinfty_i)(\pstate) >  (\iverson{\bp_j}\cdot \eainfty_j)(\pstate) 
%   \tag{de Morgan}\\
%   %
%   %
%   \text{iff} \qquad & \smtentails{\ff}{\fg}~\text{is unsatisfiable}
%   \tag{both the $\bb_i$ and the $\bp_j$ partition the state space, see below} \\
%\end{align*}
%%
%Notice that employing $\smtinfty$ to encode $\infty$ is correct, since $\smtinfty$ is unconstrained and can thus be assigned an arbitrarily large natural number.
%\kbcommentinline{Outdated end.}
%%

We thus obtain a decision procedure for quantitative entailments in $\Elin$:
%
\begin{theorem}
	\label{thm:entailment_elin}
	Quantitative entailment in $\Elin$ is decidable.
\end{theorem}
%

%
%
\kbcommentinline{Prove incompleteness of $k$-induction (cf.\ WhatsApp Group)}
\kbcommentinline{Complexity?}

==> k_induction_algorithm.tex <==
	\begin{algorithm}[t]
		%\setstretch{2}
		\caption{Latticed $k$-induction}
		\label{alg:k_induction}
		\SetKwInput{Input}{input}\SetKwInOut{Output}{output}\SetNoFillComment
		\Input{$\laop\colon \laset \to \laset$ and $\laf \in \laset$.}
        \Output{\enquote{$\verify$} if $\laf$ is a $k$-inductive invariant, diverge otherwise.}
		%
		$\lag \leftarrow \laf$ \;
		%
        \While{$\lapp{\lag} \not\laord \laf$}{
			%
			$\lag \leftarrow \kindop{\laf}(\lag)$ \;
			%
		}
		%
		\Return $\verify$ \;		
	\end{algorithm}


==> k_induction_probabilistic_programs.tex <==
\subsection{$k$-Induction for Probabilistic Programs}
%
%
%Recall that $(\E, \, \leq)$ is a complete lattice. 
Recall that $\leq$ on expectations is the point-wise lifting of $\leq$ on non-negative extended reals. Hence, the greatest lower bound $\ff \sqcap \fg$ of $\ff, \fg \in \E$ is the point-wise minimum of $\ff$ and $\fg$, i.e.,
%
\[
   \ff \sqcap \fg \eeq \ff \emin \fg \ddefeq \lambda \pstate \mydot \min \{\ff(\sigma), \fg(\sigma) \}~.
\]
%
This and Section~\ref{sec:k_induction} give us $k$-induction for probabilistic programs:
%
\begin{corollary}
	Let $\cc = \WHILEDO{\bb}{\cc'} \in \pgcl$ and $\ff, \fg \in \E$. Furthermore, let 
	%
	\[
	\kindop{\fg} \colon \E \to \E, \qquad \fh \mapsto \charwp{\bb}{\cc'}{\ff}(\fh)  \emin \fg
	\]
	%
	be the $k$-induction operator for $\fg$ and $\charwp{\bb}{\cc'}{\ff} $. If there is $k \in \Nats$ with
	%
	\[
	   \charwp{\bb}{\cc'}{\ff}(\kindopfold{\fg}{k}(\fg)) \lleq \fg, \qquad \text{then}\qquad \wp{\cc}{\ff} \lleq \fg~.
	\]
\end{corollary}
%
\begin{proof}
	This is an immediate consequence of Corollary~\ref{cor:k_induction}.
\end{proof}
%
If $\charwp{\bb}{\cc'}{\ff}(\kindopfold{\fg}{k}(\fg)) \leq \fg$, we say that $\wp{\cc}{\ff} \leq \fg$ is is provable by $(k+1)$-induction. Similarly, we say that a $\propspacesymb$-property $(\cc, \ff, \fg)$ is $k$-inductive if $\wp{\cc}{\ff} \leq \fg$ is provable by $k$-induction. 
%
%
\begin{definition}
	Let $\propspacesymb = \propspace{\SyntE}{\pgclparam{\aexp}{\bexp}}$ be a property space. We say that
	%
	%\begin{itemize}
	%\item
	$\propspacesymb$ \emph{admits $k$-induction}, if the set 
	%
	\begin{align*}
	\big\{ (\cc, \ff, \fg) ~\mid~ (\cc, \ff, \fg)~\text{is a $k$-inductive $\propspacesymb$-property for some $k$} \big\}
	\end{align*}
	%
	is semi-decidable. \hfill $\triangle$
	%\end{itemize}
\end{definition}
%
%
\begin{theorem}
	\label{thm:admissibility_k_induction}
	%
	A property space $\propspacesymb = \propspace{\SyntE}{\pgclparam{\aexp}{\bexp}}$ admits $k$-induction, if $\propspacesymb$ admits BMC and minima of expectations are computable in $\SyntE$, i.e, there is an algorithm that on input $\ff,\fg \in \SyntE$ computes an expectation $\fh \in \SyntE$ with
	%
	\[
          \fh \eequiv \ff \emin \fg~.
	\]
	%
\end{theorem}
%
\begin{proofidea}
  The argument is similar to the proof of Theorem~\ref{thm:admissibility_bmc}. Let $\prop{\cc}{\ff}{\fg}$ be a $k$-inductive $\propspacesymb$-property for some $k$.
   The fact that $\SyntE$ is closed under $\emin$ implies that $\kindopfold{\fg}{k}(\fg)$ is computable and an element of $\SyntE$ for every $k \geq 0$. Hence, Algorithm~\ref{alg:k_induction} is the sought-after semi decision procedure.
\end{proofidea}

==> keywords.tex <==
\lstset{
    language=C,%
    %numbers=left,%
    %stepnumber=4,%
    alsoletter={<,>,:=,[,],.},
    morekeywords={
            skip,%
            new,%
            free,%
            call,%
            var,%
            procedure,%
            uniform,%
            [0.5],%
    },%
    basicstyle=\footnotesize\ttfamily,%
    keywordstyle=\bfseries,%
    commentstyle=\itshape,%
}%


==> linear_pgcl.tex <==
% !TEX root = ./main.tex

%\section{Linear Fragment of the Probabilistic Guarded Command Language}




For $\mathbb{A} \in \{\Nats, \PosRats\}$, \emph{linear arithmetic expressions} $\ee \in \aexplinpar{\mathbb{A}}$ adhere to the grammar
%
\begin{align*}
\ee \qqlongrightarrow 	
   %
   %
   & c \in \mathbb{A}  \tag{constants} \\
   %
   \qmid & x \in \Vars  \tag{$\Nats$-valued variables}\\
   %
   %
   \qmid & c \cdot \ee  \tag{multiplication by $\mathbb{A}$-valued constants}\\
   %
   %
   \qmid & \ee+\ee  \tag{addition}\\
   %
   %
   \qmid & \ee \monus \ee~. \tag{subtraction truncated at $0$ (\enquote{monus})}
\end{align*}
%
%Multiplying by constants, i.e., $n \cdot \ee$ for $n\in\Nats$ is syntactic sugar.
Furthermore, we define \emph{extended linear arithmetic expressions} 
%
\[
   \extaexplinpar{\mathbb{A}} \ddefeq \aexplinpar{\mathbb{A}} \cup \{\infty\}
\]
%
and denote these by $\eeinfty,\eainfty$ or variations.
 %We denote by $\eeinfty$ (or $\eainfty$) \emph{extended linear arithmetic expressions}, which are %linear  arithmetic expressions or $\infty$, i.e., elements of $\aexplinpar{\mathbb{A}} \cup \{\infty\}$.

We denote by $\ee(\pstate)$ the value $\ee$ evaluates to on state $\pstate$, which is defined in the standard way. The monus operation deserves special attention. We define
%
 \[
    (\ee_1 \monus \ee_2)(\pstate) \ddefeq 
    \begin{cases}
    	\ee_1(\pstate) - \ee_2(\pstate), &\text{if}~\ee_2(\pstate) \leq \ee_1(\pstate) \\
    	%
    	0, &\text{otherwise}~.
    \end{cases}
 \]
%
%

\noindent
For $\mathbb{A} \in \{\Nats, \PosRats\}$, \emph{linear Boolean expressions} $\bb \in \bexplinpar{\mathbb{A}}$ adhere to the grammar
%
\begin{align*}
\bb \qqlongrightarrow 	
   %
   %
   & \ee < \ee  \tag{strict inequality of arithmetic expressions in $\aexplinpar{\mathbb{A}}$} \\
   %
   %
   \qmid & \bb \wedge \bb \tag{conjunction} \\
   %
   %
   \qmid & \neg \bb~. \tag{negation}
\end{align*}
%
Syntactic sugar is $\false$, $\true$, $\bb \vee \bp$, $\bb \implies \bp$, $\ee_1 = \ee_2$, and $\ee_1\leq \ee_2$.

We denote by $\bb(\pstate)$ the truth value $\bb$ evaluates to on state $\pstate$, which is defined in the standard way.
We now define the set $\pgclin$ of \emph{linear $\pgcl$ programs} by
%
 \[
    \pgclin \ddefeq \pgclparam{\aexplinn}{\bexplinn}~.
 \]
%
%\mccommentinline{Is the assumption on linearity substantial to our approach? Or it depends merely on the capability of the underlying SMT solvers?}
%\kbcommentinline{The assumption of linearity results in a linear SMT encoding. In theory, you can allow for non-linear stuff but then your SMT encoding %becomes non-linear, too.}
%
%\begin{align*}
%\cc \qqlongrightarrow  &\WHILEDO{\bb}{\cc'} \tag{while loop} \\
%%
%\phantom{aa} \\
%%
%	\cc' \qqlongrightarrow 	
%	%
%	%
%	& \SKIP	\tag{effectless program} \\
%	%
%	& \qmid  \ASSIGN{x}{\ee}  \tag{assignment}\\
%	%
%	& \qmid \COMPOSE{\cc'}{\cc'} \tag{sequential composition}\\
%	%
%	& \qmid  \PCHOICE{\cc'}{p}{\cc'} \tag{probabilistic choice}\\
%	%
%	& \qmid  \ITE{\bb}{\cc'}{\cc'}~, \tag{conditional choice}
%	%
%\end{align*}
%%
%where
%%
%%\begin{itemize}
%	%\item 
%	$x \in \Vars$ is a program variable,
%	%
%	%\item 
%	$\ee \in \aexplin$ is a linear arithmetic expression,
%	%
%	%\item 
%	$p \in [0,1] \cap \Rats$ is a rational probability, and
%	%
%	%\item 
%	$\bb \in \bexplin$ is a linear Boolean expression also referred to as \emph{guard}. 
%	%Given $\cc = \WHILEDO{\bb}{\cc'} \in \pgclin$, we call $\cc'$ the \emph{(loop) body} of $\cc$. 
%\end{itemize}
%
%
%\mccommentinline{Can $p$ be a function over $\Vars$?}
%\kbcommentinline{In prinicple, yes. But again, this would result in a non-linear SMT encoding.}
%A \emph{(program) state} $\sigma \colon \Vars \to \Nats$ is a map from program variables to natural numbers. We denote the set of all states by $%\States$. Given an arithmetic expression $\ee$ (resp.\ a boolean expression $\bb$), we denote by $\sigma(\ee) \in \Nats$ (resp.\ $\sigma(\bb) \in \{% %\true, \false\}$) the evaluation of $\ee$ (resp.\ $\bb$) under $\sigma$. Given a program variable $x$ and an arithmetic expression $\ee$, we denote by
%\mccommentinline{Why $\Nats$?}
%\kbcommentinline{Suppose we allowed for negative valuations of the program variables. Now consider the postexpectation $\FF = x = \lambda \sigma %\mydot \sigma(x)$. There are (at least) two issues: First, this postexpectation is not well-defined since it is no map to \emph{non-negative} reals or inifnity. Second, if you allow for expectations that might become negative, you run into definedness issues. See Benjamin's work on Mixed-Sign Expectations~\cite{mixed_sign}. I would like to avoid both issues.}
%\mccommentinline{Yes, indeed. But I should have been more specific about the question here: Why can't we go for $\sigma \colon \Vars \to \PosReals$? This seems of help to avoid the mixed integer-real-arithmetic reasoning in the SMT encodings.}
%

%the \emph{update} of $x$ by $\ee$ in $\sigma$. 



==> outdated/problem_approach.tex <==
\section{Problem Statement and Approach}

\subsection{Problem Statement}
 Using an SMT solver and the weakest preexpectation calculus, develop an algorithm for the following problem: Let $\WHILEDO{\bb}{\cc} \in \pgcl$ be a loop with loop-free body $c$, let $\ff \in \Elin$  be a linear postexpectation, and let $\fu \in \Elin$ be a candidate upper bound. Verify or refute:
%
\[
		\wp{\WHILEDO{\bb}{\cc}}{\ff} \lleq \fu~.
\]
%
Without interpolation or $k$-induction, i.e.\ pure BMC, we cannot verify the above but only refute.
This is still quite exciting since the SMT solver neither cares about whether the loop under consideration yields an \emph{infinite-state} Markov chain or whether the set of states $\Pi$ is infinite or not
(since we represent $\Pi$ by means of a formula such as $x > 3$). We call $\bmcinst{\WHILEDO{\bb}{\cc}}{\ff}{\fu}$
a \emph{BMC instance}.

\subsection{The Idea}
\newcommand{\goal}{\textsf{goal}}
\newcommand{\goalpost}{\iverson{\goal}}
The idea of our BMC approach is simple but realizing it is non-trivial. It is closely related to value iteration and standard BMC. We first describe the high-level idea.
After that, we consider an example.

For simplicity, we focus on reachability probabilities. An extension for expected outcomes is straightforward.
Fix a BMC instance $\bmcinst{\WHILEDO{\bb}{\cc}}{\goalpost}{\fu}$. Since our postexpectation $\goalpost$ is (the Iverson bracket of) a boolean expression, $\wp{\WHILEDO{\bb}{\cc}}{\goalpost}(\sigma)$ is \emph{the probability} that the loop $\WHILEDO{\bb}{\cc}$ terminates in a final state $\sigma'$ that satisfies $\goal$ when executed on the initial state $\sigma$. Since we focus on refutation, our BMC instance thus poses the question:
%
\[
    \text{Is there a state $\sigma \in \Pi$ such that $\wp{\WHILEDO{\bb}{\cc}}{\goalpost}(\sigma) > \fu(\sigma)$ ?}
\] 
%
That is, we ask whether for every  initial state, expectation $\fu$ is an upper bound on the probability to reach a state satisfying $\goal$. 

Now consider the $\wpsymbol$-characteristic functional $\charwp{\bb}{\cc}{\goalpost}$.
We make use of the fact that for every $n \in \Nats$ and every state $\sigma$,
%
\begin{center}
		$\charwpn{\bb}{\cc}{\goalpost}{n+1}(\constexp{0}) (\sigma)
		~\text{is the probability that $\WHILEDO{\bb}{\cc}$}$ \\
		 $\text{terminates in a state satisfying $\goal$ after at most $n$ iterations on initial state $\sigma$.}$
\end{center}
%
In particular, $\charwpn{\bb}{\cc}{\goalpost}{n}(\constexp{0}) $ is an (increasingly more precise) \emph{underapproximation}
of $\wp{\WHILEDO{\bb}{\cc}}{\goalpost}$ for every $n \in \Nats$. Hence, if we are able to
%
\begin{enumerate}
	\item Compute $\charwpn{\bb}{\cc}{\goalpost}{n}(\constexp{0})$ for increasing $n \in \Nats$, and
	%
	\item check whether there is a $\sigma \in \States$ with $\charwpn{\bb}{\cc}{\goalpost}{n}(\constexp{0})(\sigma) > \fu(\sigma)$,
\end{enumerate}
%
we obtain a semi-algorithm for solving the BMC instance since:
%
\begin{theorem}
	\label{thm:n_exsists}
	Let $\bmcinst{\WHILEDO{\bb}{\cc}}{\ff}{\fu}$ be a BMC instance. Furthermore, assume that
	there is a state $\sigma \in \States$ with
	%
	\[
	 \wp{\WHILEDO{\bb}{\cc}}{\ff}(\sigma) ~{}>{}~ \fu(\sigma)~.
	\]
	%
	Then there is an $n \in \Nats$ such that
	%
	\[
	   \charwpn{\bb}{\cc}{\ff}{n}(\constexp{0})(\sigma) ~{}>{}~ \fu(\sigma)~.
	\]	
\end{theorem}
%
\begin{proof}
Assume the contrary, i.e.\ assume
%
\[
   \forall n \in \Nats \colon \charwpn{\bb}{\cc}{\ff}{n}(\constexp{0})(\sigma) \lleq \fu(\sigma)~.
\]
%
In other words, $\fu(\sigma)$ is an upper bound on 
%
\[
\setcomp{\charwpn{\bb}{\cc'}{\ff}{n}(\constexp{0})(\sigma)}{n \in \Nats} 
\]
%
and hence $\fu(\sigma)$ is equal to or greater than the \emph{least} upper bound (the supremum) of the above set, which yields
%
\[
  \sup_{n \in \Nats} \setcomp{\charwpn{\bb}{\cc'}{\ff}{n}(\constexp{0})(\sigma)}{n \in \Nats}
  \eeq \wp{\WHILEDO{\bb}{\cc}}{\ff}(\sigma) 
  \lleq \fu(\sigma)~.
\]
%
This contradicts our assumption.
\end{proof}
%
From a high-level perspective, the algorithm proceeds similar to standard SAT- or SMT-based BMC:
%
\begin{enumerate}
	\item Initialize $n \leftarrow 1$
	%
	\item Push the first formula $F_1$ describing $\charwpn{\bb}{\cc}{\ff}{1}(\constexp{0})$ onto the solver.
	%
	\item Loop:
	%
	\begin{enumerate}
        \item Check via SMT query whether there is a state $\sigma \in \States$ with 
        %
        \[
              \charwpn{\bb}{\cc}{\ff}{n}(\constexp{0})(\sigma) ~{}>{}~ \fu(\sigma)~.
        \]
        %
        \item If SAT, then return REFUTE. 
        %
        \item Push formula $F_{n+1}$ (which refers to $F_n$) describing $\charwpn{\bb}{\cc}{\ff}{n+1}(\constexp{0})$ onto the solver.
        %
        \item Set $n \leftarrow n+1$.
	\end{enumerate}
\end{enumerate}
%
By Theorem~\ref{thm:n_exsists}, this algorithm semi-decides the BMC instance.



\subsection{Example}
\kbcommentinline{Outdated. Still contains state set $\Pi$.}
\newcommand{\chainprog}{\textit{chain}\xspace}

\input{chain_tikz}

Let us consider a simple example program coined \chainprog:
%
\begin{align*}
   &\WHILE{count < 5 \wedge f = \false} \\
   %
   & \quad \PCHOICE{\ASSIGN{count}{count+1}}{0.8}{\ASSIGN{f}{\true}} \\
   %
   &\}
\end{align*}
%
Denote the loop body by $c'$.
Furthermore, let $\Pi = \statepred{count=0, f=\false}$, $\ff = \iverson{f=\true}$, and $\fu = \constexp{0.3}$. Here $\statepred{count=0, f=\false}$ is a state predicate characterizing the set of states
%
\[
   \statepred{count=0, f=\false} \eeq \setcomp{\sigma \in \States}{\sigma(count)=0 \wedge \sigma(f) = \false}~.
\]
%
Notice that this state predicate covers all variables occurring in program \chainprog and can therefore be regarded as describing \emph{a single} initial state: Two states in $\statepred{count=0, f=\false}$ can only differ for those variables that do not occurr in \chainprog and therefore coincide w.r.t.\ to \chainprog.

We just described a concrete BMC instance $\bmcinst{\WHILEDO{\bb}{\cc}}{\iverson{f=\true}}{\constexp{0.3}}$. Let $\sigma_0 \in \States$ with $\sigma_0 (count) = 0$ and $\sigma_0 (f) = \false$. 
A reachable fragment of the MC corresponding to \chainprog with initial state $\sigma_0$ is depicted in Figure~\ref{fig:mc_chain_prog}. States satisfying $f=\true$ are marked with double lines.  Our algorithm is supposed to answer the question
%
\[
     \text{is $\wp{\chainprog}{\iverson{f = \true}}(\sigma_0) ~{}>{}~\constexp{0.3}(\sigma_0) \eeq 0.3$ ?}
\]
%
The answer is \emph{yes} since $\wp{\chainprog}{\iverson{f = \true}}(\sigma_0) = 0.67232 > 0.3$. Let's see how our algorithm discovers this.

For that, we first determine the $\wpsymbol$-characteristic functional:
%
\begin{align*}
%
   &\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\fg) \\
   \eeq & \iverson{count < 5 \wedge f = \false} \cdot \wp{c'}{\fg} + \iverson{\neg (count < 5 \wedge f = \false)} \cdot \iverson{f=\true} \\
   %
   \eeq & \iverson{count < 5 \wedge f = \false} \cdot \wp{\PCHOICE{\ASSIGN{count}{count+1}}{0.8}{\ASSIGN{f}{\true}}}{\fg} \\
   & \quad  + \iverson{\neg (count < 5 \wedge f = \false)} \cdot \iverson{f=\true} \\
   %
   \eeq & \iverson{count < 5 \wedge f = \false} \cdot \big(
   0.8 \cdot \wp{\ASSIGN{count}{count+1}}{\fg} +
   	0.2 \cdot \wp{\ASSIGN{f}{\true}}{\fg} \big) \\
   & \quad  + \iverson{\neg (count < 5 \wedge f = \false)} \cdot \iverson{f=\true} \\
   %
   \eeq & \iverson{count < 5 \wedge f = \false} \cdot \big(
   0.8 \cdot \fg \subst{count}{count+1} +
   0.2 \cdot \fg\subst{f}{\true} \big) \\
   & \quad  + \iverson{\neg (count < 5 \wedge f = \false)} \cdot \iverson{f=\true} \\
   %
   \eeq & \iverson{count < 5 \wedge f = \false} \cdot \big(
   0.8 \cdot \fg \subst{count}{count+1} +
   0.2 \cdot \fg\subst{f}{\true} \big) \\
   & \quad  + \iverson{f=\true} \\
%
\end{align*}
%
Let us rewrite $\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\fg)$ furhter  in a form we will later coin \emph{summation normal form}:
%
\begin{align*}
   %
   &\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\fg)  \\
   %
   \eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot \fg \subst{count}{count+1} \\
   & + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot \fg\subst{f}{\true} \\
   & + \iverson{f=\true}\\
   %
   %
\end{align*}
%
%
Now recall that 
%
\begin{center}
	$\charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n+1}(\constexp{0}) (\sigma)
	~\text{is the probability that}$ \\
	$\text{$\WHILEDO{count < 5 \wedge f = \false}{\cc'}$ terminates in a state satisfying $\iverson{f=\true}$}$ \\
	$\text{after at most $n$ iterations on initial state $\sigma$.}$
\end{center}
%
Let's gain some intuition.
%
We have
%
\begin{align*}
   & \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{1}(\constexp{0}) 
   %
   \eeq  \iverson{f=\true} \eeq \lambda \sigma \mydot 
   \begin{cases}
      1, & \text{if}~\sigma(f) = \true \\
      0, &\text{otherwise}~.
   \end{cases}
\end{align*}
%
This makes sense: The probability to reach a final state satisfying $f=\true$ in $0$ steps is $1$ if we execute the program on a state with $f=\true$, and $0$ for all other states. We now check whether
%
\[
   \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{1}(\constexp{0}) (\sigma_0)
   \eeq \iverson{f=\true}(\sigma_0)
   \eeq 0 ~{}>{}~0.3~,
\]
%
which is not the case.

We thus continue by calculating:
%
\begin{align*}
  & \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{2}(\constexp{0}) \\
  %
  \eeq& \charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}
  (\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\constexp{0})) \\
  %
  \eeq&\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\iverson{f=\true}) \\
  %
  \eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot \iverson{f=\true} \subst{count}{count+1} \\
  & + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot \iverson{f=\true}\subst{f}{\true} \\
  & + \iverson{f=\true} \\
  %
  \eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot \iverson{f=\true} \\
  & + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot \iverson{\true=\true} \\
  & + \iverson{f=\true} \\
  %
   \eeq & \phantom{{}+{}} 0.2\cdot \iverson{count < 5 \wedge f = \false} \\
  & + \iverson{f=\true}
  \tag{since $\iverson{\true = \true} = \constexp{1}$ and $\iverson{f=\false} \cdot \iverson{f=\true} = \constexp{0}.$}
  %
\end{align*}
%
Again, this makes sense: For states satisfying $f= \true$, the probability to reach a final state satisfying $f=\true$ in at most $1$ step remains $1$. By looking at Figure~\ref{fig:mc_chain_prog}, we also see
that the probability to reach a final state satisfying $f=\true$ from some state satisfying $count<5 \wedge f = \false$ in at most $1$ step is $0.2$. Again, we check whether
%
\[
   \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{2}(\constexp{0})(\sigma_0)
   \eeq 0.2 ~{}>{}~0.3~,
\]
%
which is not the case.

We perform one final iteration. Proceeding in a less detailed manner, we calculate:
%
%
\begin{align*}
& \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{3}(\constexp{0}) \\
%
\eeq& \charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}
(\charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{2}(\constexp{0}))  \\
%
\eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot (0.2\cdot \iverson{count < 5 \wedge f = \false}  + \iverson{f=\true}) \subst{count}{count+1} \\
& + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot (0.2\cdot \iverson{count < 5 \wedge f = \false}  + \iverson{f=\true})\subst{f}{\true} \\
& + \iverson{f=\true}\\
%
\eeq & \phantom{{}+{}} 0.8 \cdot 0.2 \cdot \iverson{count < 5 \wedge f = \false}  \cdot  \iverson{count < 4 \wedge f = \false} \\
& + 0.2 \cdot \iverson{count < 5 \wedge f = \false} \\
& + \iverson{f=\true}\\
%
\eeq & \phantom{{}+{}} 0.8 \cdot 0.2 \cdot \iverson{count < 4 \wedge f = \false}  \\
& + 0.2 \cdot \iverson{count < 5 \wedge f = \false}  \\
& + \iverson{f=\true}\\
%
%
\end{align*}
%
This expectation now expresses for every state the probability to reach a final state with $f=\true$ in at most $2$ steps. For the state $count=4 \wedge f=\false$, this probability is still $0.2$ (convince yourself by means of Figure~\ref{fig:mc_chain_prog}). For every state with $count<4 \wedge f=\false$, this probability is $0.8*0.2+0.2$. Finally, we check whether
%
\[
  \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{3}(\constexp{0})(\sigma_0)
  \eeq 0.8\cdot0.2+0.2 \eeq 0.36 ~{}>{}~0.3~
\]
%
is satisfiable,
which is the case. Hence, we have performed enough unfoldings of the $\wpsymbol$-characteristic functional to prove that $\constexp{0.3}$ is not an upper bound on the weakest preexpectation we are interested in for the state $\sigma_0$.
We have not only gained intuition on what it means to iterate the $\wpsymbol$-characteristic functional, but we also see that---even for such a simple example---it is quite cumbersome to perform this iteration. This is definitely something we want to automate.

\subsection{SMT Encoding by Example}
\label{sec:smt_encoding_example}
\newcommand{\varval}[1]{\textsf{val}_{#1}}

We now describe how to encode our problem by means of logical formulae. We first describe an encoding involving quantifiers. Since quantifiers slow down the SMT solver significantly, we then show how to obtain an equisatisfiable and quantifier-free SMT encoding.

Our first encoding lives in the combined theory \textsf{UF\_LRIA} of uninterpreted functions \footnote{\url{https://en.wikipedia.org/wiki/Uninterpreted_function}} and linear real- and integer arithmetic, where we
\mccommentinline{Due to Weispfenning~\cite{DBLP:conf/issac/Weispfenning99}, the theory of linear, multivariate mixed real-integer arithmetic is known to be decidable and admit quantifier elimination. Better clarify if the decidability remains with EUF.}
%
\begin{itemize}
   \item use uninterpreted functions to represent expectations,
   %
   \item use integer arithmetic to represent program states, and
   %
   \item use real arithmetic to represent probabilities and expected outcomes, i.e.\ the codomain of expectations.
\end{itemize}
%
Recall that we represent the $\wpsymbol$-characteristic functional of our example in summation normal form:
%
\begin{align*}
%
&\charwp{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}(\fg)  \\
%
\eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot \fg \subst{count}{count+1} \\
& + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot \fg\subst{f}{\true} \\
& + \iverson{f=\true}\\
%
%
\end{align*}
%
We thus have for every $n \in \Nats$,
%
\begin{align}
%
&\charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n+1}(\constexp{0})
 \label{eqn:phi_n_dependency} \\
%
\eeq & \phantom{{}+{}} 0.8 \cdot \iverson{count < 5 \wedge f = \false}  \cdot \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n}(\constexp{0}) \subst{count}{count+1} 
\notag \\
%
& + 0.2\cdot \iverson{count < 5 \wedge f = \false}\cdot \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n}(\constexp{0})\subst{f}{\true}
\notag \\
%
& + \iverson{f=\true} ~.
\notag 
%
%
\end{align}
%
From now on, we assume for every $n > 0$ an uninterpreted function $P_n$ of type $\Ints \times \Ints \to \Reals$. The goal of our SMT encoding is to maintain the followin \emph{loop invariant}: At the beginning of the $n$th iteration of our algorithm, we have for every state $\sigma$ and every $\delta \in [0,1]$:
%
\begin{align*}
	&\text{current\_set\_of\_formulae}~\wedge~P_n(\sigma(count), \sigma(f)) > \lambda\quad \text{is satisfiable} \\
	\text{iff} \quad &
	\charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n}(\constexp{0}) (\sigma) > \delta~.
\end{align*}
%
As suggested by Equation~\ref{eqn:phi_n_dependency}, the formula $F_{n+1}$ defining $P_{n+1}$ will refer to the formula $F_n$ defining $P_n$. At the beginning of the $n$th iteration, we have
%
\[
  \text{current\_set\_of\_formulae} \eeq \bigwedge_{i=1}^n F_n~.
\]
%
\noindent
\emph{The first formula $F_1$.} Recall that 
%
\begin{align*}
& \charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{1}(\constexp{0}) 
%
\eeq  \iverson{f=\true} \eeq \lambda \sigma \mydot 
\begin{cases}
1, & \text{if}~\sigma(f) = \true \\
0, &\text{otherwise}~.
\end{cases}
\end{align*}
%
Hence,
%
\begin{align*}
   F_1 \eeq & \forall count \in  \Ints \colon \forall f \in \Bools \colon \\
   & \quad (f =\true \implies P_1(count, f) = 1)
    \quad ~{}\wedge{}~ 
    (f \neq \true \implies P_1(count, f) = 0)~.
\end{align*}
%
It is quite easy to see that this fulfills our loop invariant at the beginning of the loop.
Notice, however, that we have to explicitly encode that $P_1(count, f)$ evaluates to $0$ if $f \neq \true$. \\ \\
%
\noindent
\emph{Encoding the formuila $F_{n+1}$.} Now assume that we pushed all formulae $F_i$ for $i = 1,\ldots,n$ onto the solver. Inspired by Equation~\ref{eqn:phi_n_dependency}, we now push
%
\begin{align*}
	F_{n+1} \eeq&   \forall count \in  \Ints \colon \forall f \in \Bools \colon \\
	%
	& \phantom{{}\wedge{}}\qquad (count < 5 \wedge f =\false) ~{}\implies{}~ P_{n+1}(count, f) = 0.8 \cdot P_n(count +1, f) + 0.2 \cdot P_n (count, \true)  \\
	%
	& \wedge \qquad f=\true ~{}\implies{}~ P_{n+1}(count, f) = 1 \\
	%
	&\wedge \qquad  \neg(count < 5 \wedge f =\false) \wedge \neg(f=\true )
	~{}\implies{}~ P_{n+1}(count, f) = 0~.
\end{align*}
%
onto the solver. Notice how substitutions like $\fg\subst{count}{count+1}$ and $\fg\subst{f}{\true}$ translate to $P_n(count +1, f)$ and $P_n (count, \true) $, respectively. \\ \\
%
\noindent
%
Observe that I have cheated a bit. I exploited that the boolean expressions occurring in the first two summands of $\charwpn{count < 5 \wedge f = \false}{\cc'}{\iverson{f=\true}}{n+1}(\constexp{0})$ are equivalent (and in fact coincide syntactically). Without optimizations, our algorithm does not see this. 

Now consider the more general case where we are given a loop $ c = \WHILEDO{\bb}{\cc'}$, some postexpectation $\ff$ and where the program variables occurring in $c$ and $\ff$ are $x_1,\ldots,x_u$. Suppose that the $\wpsymbol$-characteristic functional in summation normal form is given by
%
\[
   \charwp{\bb}{c'}{\ff}(\fg) \eeq 
   \iverson{\neg \bb} \cdot \ff  ~{}+{}~ 
   \sum_{i=1}^{m} prob_i \cdot \bb_i 
      \cdot \fg\left[ x_1 / \textsf{upd}_{1,i}, \ldots, x_u  / \textsf{upd}_{u,i} \right] ~.
\]
%
We have to take into account that the $b_i$ are not necessarily mutually exclusive, i.e.\ that they might \enquote{overlap} (cf.\ Equation~\ref{eqn:phi_n_dependency}). In this general setting, formula $F_{n+1}$ is thus given by
%
\begin{align*}
  F_{n+1} \eeq& \forall x_1, \ldots, x_u \colon  \neg \bb \implies P_{n+1}(x_1,\ldots,x_u) = \ff(x_1,\ldots,x_u) \\
  &\quad \wedge \bigwedge_{((B_i, Prob_i)_{1\leq i \leq m}) \in \bigtimes_{j=1}^{m} \{ (\bb_j, prob_j) , (\neg \bb_j, 0)\}} 
  \Big( \bigwedge_{i=1}^{m} B_i \\
  &\qquad \qquad \qquad \qquad \qquad \qquad ~{}\implies{}~ 
  		P_{n+1}(x_1,\ldots,x_u) = \sum_{i=1}^{m} Prob_i \cdot P_n(\textsf{upd}_{1,i}, \ldots, \textsf{upd}_{u,i}) \Big) ~.
   %
\end{align*}
%
Since $|\bigtimes_{j=1}^{m} \{ (\bb_j, prob_j) , (\neg \bb_j, 0)\}| = 2^m$, we have an exponential blow-up in the number of summands of the $\wpsymbol$-characteristic functional for every formula $F_{n+1}$. An appropriate preprocessing can mittigate this significantly. Every $((B_i, Prob_i)_{1\leq i \leq m}) \in \bigtimes_{j=1}^{m} \{ (\bb_j prob_j) , (\neg \bb_j, 0)\}$ where $\bigwedge_{i=1}^{m} B_i$ is unsatisfiable can be disregarded.
%
%
\subsection{Towards an Equisatisfiable, Quantifier-Free Encoding}

We investiagte a quantifier-free encoding. Let us first see what happens if we simply drop the quantifiers to understand why we need the quantifiers in our current encoding.
Consider the formulae $F_1$ and $F_2$ for our chain example:
%
%
\begin{align*}
F_1 \eeq & \forall count \in  \Ints \colon \forall f \in \Bools \colon \\
& \quad (f =\true \implies P_1(count, f) = 1)
\quad ~{}\wedge{}~ 
(f \neq \true \implies P_1(count, f) = 0) \\
%
F_{2} \eeq&   \forall count \in  \Ints \colon \forall f \in \Bools \colon \\
%
& \phantom{{}\wedge{}}\qquad (count < 5 \wedge f =\false) ~{}\implies{}~ P_{2}(count, f) = 0.8 \cdot P_1(count +1, f) + 0.2 \cdot P_1 (count, \true)  \\
%
& \wedge \qquad f=\true ~{}\implies{}~ P_{2}(count, f) = 1 \\
%
&\wedge \qquad  \neg(count < 5 \wedge f =\false) \wedge \neg(f=\true )
~{}\implies{}~ P_{2}(count, f) = 0~.
\end{align*}
%
We introduce free variables $count$ and $f$ with domain $\Ints$ and $\Bools$, respectively, and obtain:
%
\begin{align*}
F_1' \eeq & \\
& \quad (f =\true \implies P_1(count, f) = 1)
\quad ~{}\wedge{}~ 
(f \neq \true \implies P_1(count, f) = 0) \\
%
F_{2}' \eeq&   \\
%
& \phantom{{}\wedge{}}\qquad (count < 5 \wedge f =\false) ~{}\implies{}~ P_{2}(count, f) = 0.8 \cdot P_1(count +1, f) + 0.2 \cdot P_1 (count, \true)  \\
%
& \wedge \qquad f=\true ~{}\implies{}~ P_{2}(count, f) = 1 \\
%
&\wedge \qquad  \neg(count < 5 \wedge f =\false) \wedge \neg(f=\true )
~{}\implies{}~ P_{2}(count, f) = 0~.
\end{align*}
%
We invoke z3 to check the satisfiability of 
%
\begin{align}
\label{form:ex_chain_1}
    F_1' ~{}\wedge{}~ F_2' ~{}\wedge{}~count=0~{}\wedge{}~f=\false~{}\wedge{}~P_2(count,f) > 0.3~.
\end{align}
%
%
A sound encoding must return UNSAT since the probability to reach $\goal$ state in at most $1$ step from $\sigma_0$ is not greater than $0.3$. However, z3 returns SAT and provides the following model:
%
%
\begin{align*}
   count \eeq& 0 \\
   %
   f \eeq& \false \\
   %
   P_1 \eeq& \lambda (count, f) \mydot 
   \begin{cases}
      \frac{13}{8}, &\text{if}~(count,f) = (1, \false) \\
      0,&\text{otherwise}
      \end{cases}\\
    %
    P_2 \eeq& \lambda (count, f) \mydot \frac{13}{10}~.
   %
\end{align*}
%
Convince yourself that this is indeed a model of Formula~\ref{form:ex_chain_1}.
What happens here? The problem is the subterm $P_1(count +1, f)$ (and $P_1(count, \true)$) in the first implication of $F_2'$. Looking at $F_1'$, we see that we tell the solver nothing about $P_1(count +1, f) $, which means that the solver may assign an arbitrary value for the function $P_1$ at these arguments to obtain a model. Without constraining $P_1(count +1, f) $ (and $P_1(count, \true)$), our encoding is therefore unsound.

\subsection{A Solution}
%
We fix this issue by pushing appropriate copies of $F_1$. Let's go through the algorithm again.
First constraints for $P_1$:
%
\begin{align*}
%
F_1 \eeq &  (f =\true \implies P_1(count, f) = 1)
\quad ~{}\wedge{}~ 
(f \neq \true \implies P_1(count, f) = 0) 
%
\end{align*}
%
The first query
%
\[
   F_1 ~{}\wedge{}~count=0~{}~\wedge{}~f=\false
   ~{}\wedge{}~P_1(count,f) > 0.3
\]
%
is unsat. Next iteration. Push the formula $F_2$ for $P_2$:
%
\begin{align*}
	F_{2} \eeq &  \phantom{{}\wedge{}}\qquad (count < 5 \wedge f =\false) ~{}\implies{}~ P_{2}(count, f) = 0.8 \cdot P_1(count +1, f) + 0.2 \cdot P_1 (count, \true)  \\
	%
	& \wedge \qquad f=\true ~{}\implies{}~ P_{2}(count, f) = 1 \\
	%
	&\wedge \qquad  \neg(count < 5 \wedge f =\false) \wedge \neg(f=\true )
	~{}\implies{}~ P_{2}(count, f) = 0~.
\end{align*}
%
We now have to push formulae constraining $P_1(count+1, f)$ and $P_1(count, \true)$.
Denote by $F_1\subst{count,f}{expr_1, expr_2}$ the formula obtained from $F_1$ by substituting every occurrence of $count$ and $f $ in $F_1$ by $expr_1$ and $expr_2$, respectively. The constraints for $P_1(count+1, f)$ and $P_1(count, \true)$ are :
%
\begin{align*}
%
   F_1\subst{count,f}{count+1,f}
   \eeq&
   (f =\true \implies P_1(count + 1, f) = 1) \\
   & \quad\wedge{}~ 
   (f \neq \true \implies P_1(count +1, f) = 0) \\
   %
   F_1\subst{count,f}{count,\true} \eeq &
   (\true=\true \implies P_1(count , \true) = 1) \\
   & \qquad \wedge{}~ 
   (\true\neq \true \implies P_1(count, \true) = 0) 
   %
\end{align*}
%
\kbcommentinline{Notice that there is some potential for optimizations: Whenever the substituition of the variables results in an unsatisfiable left-hand side of some implication, this implication can be omitted. This prohibits us from generating an exponentially increasing amount of formulae whenever this is possible.}
%
The next query
%
\begin{align*}
%
&F_1 ~{}\wedge{}~
F_1\subst{count,f}{count+1,f} ~{}\wedge{}~
F_1\subst{count,f}{count,\true} \\
%
 &~{}\wedge{}~ 
F_2 ~{}\wedge{}~
count=0~{}~\wedge{}~f=\false
~{}\wedge{}~P_2(count,f) > 0.3
%
\end{align*}
%
is unsat. There is, however, a downside of this encoding, which, I think, is unavoidable.
%
Consider the next iteration. We push $F_3$:
%
\begin{align*}
F_{3} \eeq &  \phantom{{}\wedge{}}\qquad (count < 5 \wedge f =\false) ~{}\implies{}~ P_{3}(count, f) = 0.8 \cdot P_2(count +1, f) + 0.2 \cdot P_2 (count, \true)  \\
%
& \wedge \qquad f=\true ~{}\implies{}~ P_{3}(count, f) = 1 \\
%
&\wedge \qquad  \neg(count < 5 \wedge f =\false) \wedge \neg(f=\true )
~{}\implies{}~ P_{3}(count, f) = 0~.
\end{align*}
%
Similar to the last iteration, we have to push the formulae $F_2\subst{count,f}{count+1,f}$
and $F_2\subst{count,f}{count,\true}$ to constrain $ P_2(count +1, f)$ and $P_2 (count, \true)$:
%
\begin{align*}
%
   &F_2\subst{count,f}{count+1,f} \\
\eeq&
\phantom{{}\wedge{}}\qquad (count +1 < 5 \wedge f =\false) \\
&\qquad \quad ~{}\implies{}~ P_{2}(count +1, f) = 0.8 \cdot P_1(count +1 +1, f) + 0.2 \cdot P_1 (count +1, \true)  \\
%
& \wedge \qquad f=\true ~{}\implies{}~ P_{2}(count +1, f) = 1 \\
%
&\wedge \qquad  \neg(count + 1 < 5 \wedge f =\false) \wedge \neg(f=\true )
~{}\implies{}~ P_{2}(count + 1, f) = 0 \\
%
%
\phantom{a} \\
%
&F_2\subst{count,f}{count,\true} \\
 \eeq &
\phantom{{}\wedge{}}\qquad (count < 5 \wedge \true =\false) \\
& \qquad \quad ~{}\implies{}~ P_{2}(count, \true) = 0.8 \cdot P_1(count +1, \true) + 0.2 \cdot P_1 (count, \true)  \\
%
& \wedge \qquad \true=\true ~{}\implies{}~ P_{2}(count, \true) = 1 \\
%
&\wedge \qquad  \neg(count < 5 \wedge \true =\false) \wedge \neg(\true=\true )
~{}\implies{}~ P_{2}(count, \true) = 0~.
%
%
\end{align*}
%
We thus have new occurrences of $P_1$, namely $P_1(count+1+1, f)$ and $P_1(count+1, \true)$ (notice that $P_1(count, \true)$ is already constrained). However, since the first implication in $F_2\subst{count,f}{count,\true}$ is unsatisfiable, we do not have to constrain $P_1(count+1, \true)$. On the other hand, for $P_1(count+1+1, f)$ and $P_1(count+1, \true)$, we \emph{do} have to push formulae. 
We see that our quantifier-free encoding requires us to push copies of the formulae $F_i$ for \emph{all} $i<k$ when pushing $F_k$. This is due to the fact that unrolling the $\wpsymbol$-characteristic functional requires ever more values of $P_1,P_2,\ldots$. The dependency graph depicted in Figure~\ref{fig:chain_p_dependency} underlines this. Notice the similarities between the structure of the dependency graph and the underlying Markov chain of the loop (Figure~\ref{fig:mc_chain_prog}). This is no coincidence: Unrolling the $\wpsymbol$-characteristic functional correspondonds to a \enquote{symbolic unrolling} of the underlying Markov chain.

  The number of new formulae (i.e.\ instances of the $F_i$) required for $F_k$ is in
%
\[
   O (\max \setcomp{
     \text{number of states reachable from $\sigma$ in at most $k-1$ steps}}
      {\sigma \in \Sigma}
       )~.
\]
%
Thus, in the worst case, the number of required copies of the $F_i$ grows exponentially in the number of loop iterations $k$. This is the case, e.g., if the underlying Markov chain has the structure of a complete binary tree. On the other hand, in our $\chainprog$ example,the number of required formulae grows only linearly.


\begin{figure}
	\begin{tikzpicture}
	     \node (s1) {$P_3(count, f)$};
	     
	     \node[below left=1cm and 1cm of s1] (s2) {$P_2(count +1, f)$};
	     \node[below right = 1cm and 1.5cm of s1] (s3) {$P_2(count , \true)$};
	     
	     \node[below left= 1cm and -1cm of s2] (s4) {$P_1(count +1 + 1, f)$};
	     \node[below right= 1cm and -1cm of s2] (s5) {$P_1(count +1, \true)$};
	     
	     %\node[below =1 cm of s3] (s3) {$P_1(count, \true)$};
	     
	     \draw[->] (s1) edge (s2);
	     \draw[->] (s1) edge (s3);
	     \draw[->] (s2) edge (s4);
	     \draw[->] (s2) edge (s5);
	\end{tikzpicture}
	\phantom{aa}
		\phantom{aa}
			\phantom{aa}
\begin{tikzpicture}
	\node (s1) {$P_4(count, f)$};
	
	\node[below left=1cm and 1.5cm of s1] (s2) {$P_3(count +1, f)$};
	\node[below right = 1cm and 1.5cm of s1] (s3) {$P_3(count , \true)$};
	
	\node[below left= 1cm and -0.5cm of s2] (s4) {$P_2(count +1 + 1, f)$};
	\node[below right= 1cm and -0.5cm of s2] (s5) {$P_2(count +1, \true)$};
	
	
		\node[below left= 1cm and -1cm of s4] (s6) {$P_2(count +1 + 1+1, f)$};
	\node[below right= 1cm and -1cm of s4] (s7) {$P_2(count +1+1, \true)$};

	
	%\node[below =1 cm of s3] (s3) {$P_1(count, \true)$};
	
	\draw[->] (s1) edge (s2);
	\draw[->] (s1) edge (s3);
	\draw[->] (s2) edge (s4);
	\draw[->] (s2) edge (s5);
	\draw[->] (s4) edge (s6);
		\draw[->] (s4) edge (s7);
	\end{tikzpicture}
	
	\caption{Dependency graph of the $P$s for the $\chainprog$ example.}\label{fig:chain_p_dependency}
\end{figure}
